A Contrastive Cross-Channel Data Augmentation Framework for Aspect-based Sentiment Analysis

Aspect-based sentiment analysis (ABSA) is a fine-grained sentiment analysis task, which focuses on detecting the sentiment polarity towards the aspect in a sentence. However, it is always sensitive to the multi-aspect challenge, where features of multiple aspects in a sentence will affect each other. To mitigate this issue, we design a novel training framework, called Contrastive Cross-Channel Data Augmentation (C3 DA), which leverages an in-domain generator to construct more multi-aspect samples and then boosts the robustness of ABSA models via contrastive learning on these generated data. In practice, given a generative pretrained language model and some limited ABSA labeled data, we first employ some parameter-efficient approaches to perform the in-domain fine-tuning. Then, the obtained in-domain generator is used to generate the synthetic sentences from two channels, i.e., Aspect Augmentation Channel and Polarity Augmentation Channel, which generate the sentence condition on a given aspect and polarity respectively. Specifically, our C3 DA performs the sentence generation in a cross-channel manner to obtain more sentences, and proposes an Entropy-Minimization Filter to filter low-quality generated samples. Extensive experiments show that our C3 DA can outperform those baselines without any augmentations by about 1% on accuracy and Macro- F1. Code and data are released in https://github.com/wangbing1416/C3DA.

==> Sec_Limitations.tex <==
\section{Limitations}
% We discuss the potential limitations of our work.
Indeed, our overall work has some potential limitations, and we will discuss them in this section.

\paragraph{Method}
our \baby is a flexible method, we can generate $k$ samples for each source sentence. However, an effective filtering method is vital with $k$ increasing, we follow a proposed hypothesis. It is worth investigating whether this is a reasonable assumption and whether there is a more authoritative assumption.


\paragraph{Experiment}
We have tried our best to conduct exhaustive experiments, including main experiments, ablation studies, sensitivity analyses,  and case studies. However, our baselines may be lacking, because there are so less DA-based works in the ABSA area. As alternatives, we select some DA methods in the NLU area to compare. Meanwhile, some generative DA methods need to be compared, such as \citet{Anaby2020do}, but these generative DA methods are aspect-destructive and don't have released codes. We have already considered this, \newcite{Anaby2020do} fine-tunes the whole pre-trained model to conditionally generate some sentences, so we change our fixed T5 model with parameter efficient methods to a unfixed T5 model to simulate it, more experiments are shown in Appendix \ref{AppendixA}.
